Semi-Supervised Dialogue Abstractive Summarization via High-Quality Pseudolabel Selection

Semi-supervised dialogue summarization (SSDS) leverages model-generated summaries to reduce reliance on human-labeled data and improve the performance of summarization models. While addressing label noise, previous works on semi-supervised learning primarily focus on natural language understanding tasks, assuming each sample has a unique label. However, these methods are not directly applicable to SSDS, as it is a generative task, and each dialogue can be summarized in different ways. In this work, we propose a novel scoring approach, SiCF, which encapsulates three primary dimensions of summarization model quality: Semantic invariance (indicative of model confidence), Coverage (factual recall), and Faithfulness (factual precision). Using the SiCF score, we select unlabeled dialogues with high-quality generated summaries to train summarization models. Comprehensive experiments on three public datasets demonstrate the effectiveness of SiCF scores in uncertainty estimation and semi-supervised learning for dialogue summarization tasks. Our code is available at \url{https://github.com/amazon-science/summarization-sicf-score}.

==> copy/copy_tables.tex <==
% below is for the tables
\begin{table*}[]
    \caption{SSDS results on SAMSUM 1:50. } 
    \label{tab:ssds_samsum_1_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & 43.90                                               & 18.49                                               & 35.02                                               & 0.4374                                                  \\
Use all            & 1                                                        & 44.32                                               & 19.07                                               & 35.43                                               & 0.4372                                                  \\
\hline
Random rank        & 0.5                                                      & 45.16                                               & 19.47                                               & 35.59                                               & 0.4442                                                  \\
SiCF (mean)        & 0.5                                                      & 44.98                                               & 19.25                                               & 34.98                                               & 0.4385                                                  \\
SiCF (BNN)         & 0.5                                                      & 45.07                                               & 19.18                                               & 34.95                                               & 0.4434                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 45.14                                               & 19.47                                               & 35.19                                               & 0.4440                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                      & 45.05	&19.15	&35.12	&0.4442                                                  \\
Pseudo oracle      & 0.5                                                      & 45.58                                               & 19.79                                               & 35.95                                               & 0.4400                                                  \\
\hline
Random rank        & 0.25                                                     & 44.98                                               & 19.32                                               & 35.65                                               & 0.4439                                                  \\
SiCF (mean)        & 0.25                                                     & 45.85                                               & 19.90                                               & 35.96                                               & 0.4489                                                  \\
SiCF (BNN)         & 0.25                                                     & 45.20                                               & 19.95                                               & 35.63                                               & 0.4445                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 45.14                                               & 19.31                                               & 35.59                                               & 0.4447                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 45.40	&19.38	&35.48	&0.4434                                                  \\
Pseudo oracle      & 0.25                                                     & 44.92                                               & 19.87                                               & 35.67                                               & 0.4432   
\\                                             \hline 
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on SAMSUM 5:50. } 
    \label{tab:ssds_samsum_5_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & { 46.81}                        & { 20.46}                        & { 36.38}                        & { 0.4574}                           \\
Use all            & 1                                                        & { 47.76}                        & { 21.84}                        & { 38.20}                        & { 0.4702}                           \\
\hline
Random rank        & 0.5                                                      & 47.87                                               & 21.19                                               & 37.33                                               & 0.4677                                                  \\
SiCF (mean)        & 0.5                                                      & 47.94                                               & 21.51                                               & 37.09                                               & 0.4648                                                  \\
SiCF (BNN)         & 0.5                                                      & 47.72                                               & 21.39                                               & 37.46                                               & 0.4653                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 47.98                                               & 21.77                                               & 37.72                                               & 0.4704                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 48.23	& 21.83	&37.64	&0.4663                                              \\
Pseudo oracle      & 0.5                                                      & 48.40                                               & 21.73                                               & 38.16                                               & 0.4757                                                  \\
\hline
Random rank        & 0.25                                                     & 47.65                                               & 21.13                                               & 37.18                                               & 0.4666                                                  \\
SiCF (mean)        & 0.25                                                     & 47.90                                               & 21.39                                               & 37.57                                               & 0.4651                                                  \\
SiCF (BNN)         & 0.25                                                     & 47.77                                               & 22.07                                               & 37.67                                               & 0.4635                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 48.14                                               & 22.05                                               & 37.63                                               & 0.4661                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 47.83	&21.40	&37.24	&0.4655                                                  \\
Pseudo oracle      & 0.25                                                     & 48.33                                               & 21.97                                               & 37.93                                               & 0.4732                                                 
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on DialogSUM 1:50. } 
    \label{tab:ssds_dialogsum_1_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & { 40.30}                        & { 14.53}                        & { 31.19}                        & { 0.4389}                           \\
Use all            & 1                                                        & { 39.22}                        & { 14.04}                        & { 30.50}                        & { 0.4349}                           \\
\hline
Random rank        & 0.5                                                      & 39.54                                               & 14.58                                               & 30.92                                               & 0.4401                                                  \\
SiCF (mean)        & 0.5                                                      & 40.09                                               & 14.71                                               & 31.08                                               & 0.4366                                                  \\
SiCF (BNN)         & 0.5                                                      & 40.30                                               & 14.84                                               & 31.35                                               & 0.4418                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 39.16                                               & 14.19                                               & 30.71                                               & 0.4415                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 39.61	&14.75	&31.25	&0.4422                                                  \\
Pseudo oracle      & 0.5                                                      & 40.37                                               & 14.54                                               & 31.44                                               & 0.4469                                                  \\
\hline
Random rank        & 0.25                                                     & 39.66                                               & 14.32                                               & 30.89                                               & 0.4365                                                  \\
SiCF (mean)        & 0.25                                                     & 39.56                                               & 14.18                                               & 31.02                                               & 0.4360                                                  \\
SiCF (BNN)         & 0.25                                                     & 39.48                                               & 14.27                                               & 31.26                                               & 0.4401                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 39.98                                               & 14.68                                               & 31.14                                               & 0.4392                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 39.90	&14.40	&31.44	&0.4434                                                  \\
Pseudo oracle      & 0.25                                                     & 40.44                                               & 14.98                                               & 31.73                                               & 0.4543                                               
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on DialogSUM 5:50. } 
    \label{tab:ssds_dialogsum_5_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & { 42.28}                        & { 15.61}                        & { 33.18}                        & { 0.4629}                           \\
Use all            & 1                                                        & { 41.61}                        & { 16.04}                        & { 33.25}                        & { 0.4612}                           \\
\hline
Random rank        & 0.5                                                      & 42.06                                               & 16.01                                               & 33.07                                               & 0.4614                                                  \\
SiCF (mean)        & 0.5                                                      & 41.15                                               & 15.86                                               & 32.71                                               & 0.4522                                                  \\
SiCF (BNN)         & 0.5                                                      & 41.89                                               & 15.81                                               & 33.43                                               & 0.4624                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 41.89                                               & 15.86                                               & 33.31                                               & 0.4582                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 42.33	&16.27	&33.54	&0.4649                                                  \\
Pseudo oracle      & 0.5                                                      & 42.44                                               & 16.37                                               & 33.80                                               & 0.4687                                                  \\
\hline
Random rank        & 0.25                                                     & 42.32                                               & 16.38                                               & 33.70                                               & 0.4607                                                  \\
SiCF (mean)        & 0.25                                                     & 41.77                                               & 15.87                                               & 32.79                                               & 0.4548                                                  \\
SiCF (BNN)         & 0.25                                                     & 42.00                                               & 15.95                                               & 33.47                                               & 0.4670                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 42.85                                               & 16.86                                               & 34.06                                               & 0.4645                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 43.02	&17.22	&34.32	&0.4702                                                  \\
Pseudo oracle      & 0.25                                                     & 42.71                                               & 16.10                                               & 33.77                                               & 0.4705                                       
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on TODSUM 2:90. } 
    \label{tab:ssds_todsum_2_90}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & { 76.60}                        & { 59.51}                        & { 67.87}                        & { 0.7002}                           \\
Use all            & 1                                                        & { 77.02}                        & { 59.86}                        & { 68.09}                        & { 0.7057}                           \\
\hline
Random rank        & 0.5                                                      & 77.12                                               & 60.07                                               & 68.63                                               & 0.7087                                                  \\
SiCF (mean)        & 0.5                                                      & 76.93                                               & 59.91                                               & 68.48                                               & 0.7084                                                  \\
SiCF (BNN)         & 0.5                                                      & 76.29                                               & 59.19                                               & 67.59                                               & 0.7009                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 77.06                                               & 60.78                                               & 69.10                                               & 0.7118                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 77.17	&60.39	&69.12	&0.7132                                                  \\
Pseudo oracle      & 0.5                                                      & 78.44                                               & 61.65                                               & 70.11                                               & 0.7237                                                  \\
\hline
Random rank        & 0.25                                                     & 76.91                                               & 59.43                                               & 68.29                                               & 0.7064                                                  \\
SiCF (mean)        & 0.25                                                     & 77.94                                               & 61.01                                               & 69.64                                               & 0.7172                                                  \\
SiCF (BNN)         & 0.25                                                     & 76.64                                               & 59.66                                               & 68.71                                               & 0.7053                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 77.01                                               & 59.92                                               & 69.01                                               & 0.7091                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 76.45	&59.46	&68.77	&0.7064                                                  \\
Pseudo oracle      & 0.25                                                     & 79.09                                               & 63.19                                               & 71.94                                               & 0.7396                                                 
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on TODSUM 10:90. } 
    \label{tab:ssds_todsum_10_90}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & 79.75                      & 64.69                        & 72.77                        & 0.7428                           \\
Use all            & 1                                                        & 80.00                        & 64.99                        & 73.08                        & 0.7430                           \\
\hline
Random rank        & 0.5                                                      & 80.18                                               & 65.47                                               & 73.46                                               & 0.7484                                                  \\
SiCF (mean)        & 0.5                                                      & 80.95                                               & 65.95                                               & 73.96                                               & 0.7538                                                  \\
SiCF (BNN)         & 0.5                                                      & 81.06                                               & 66.32                                               & 74.62                                               & 0.7563                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 80.76                                               & 66.29                                               & 74.29                                               & 0.7550                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 80.61	&66.25	&74.17	&0.754                                                  \\
Pseudo oracle      & 0.5                                                      & 82.49                                               & 68.48                                               & 76.40                                               & 0.7718                                                  \\
\hline
Random rank        & 0.25                                                     & 80.57                                               & 65.73                                               & 73.76                                               & 0.7513                                                  \\
SiCF (mean)        & 0.25                                                     & 81.08                                               & 66.70                                               & 74.48                                               & 0.7575                                                  \\
SiCF (BNN)         & 0.25                                                     & 82.01                                               & 67.90                                               & 75.95                                               & 0.7674                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 80.93                                               & 66.32                                               & 74.58                                               & 0.7578                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 81.22	&67.14	&75.16	&0.7615                                                  \\
Pseudo oracle      & 0.25                                                     & 83.43                                               & 70.10                                               & 77.43                                               & 0.7848                                                 
\\
\hline
\end{tabular}
\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
    \caption{Uncertainty estimation results of SiCF score three datasets (SAMSUM 1:50, DIALOGSUM 1:50 and TODSUM 2:90) in terms of Rouge-1. } 
    \label{tab:uncertainty_R1_1p}
    \centering
    \scriptsize
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{Rouge-1} & \multicolumn{2}{c|}{SAMSUM (1:50)} & \multicolumn{2}{c|}{DIALOGSUM (1:50)} & \multicolumn{2}{c}{TODSUM (2:90)} \\
                         & 0-50\% mean    & 0-90\% mean      & 0-50\% mean     & 0-90\% mean        & 0-50\% mean    & 0-90\% mean      \\ \hline
Random rank              & 58.55          & 69.62            & 56.34           & 67.97              & 82.28          & 87.04            \\
SiCF(mean)               & 59.61          & 70.83            & 57.02           & 68.65              & 83.24          & 88.00            \\
SiCF(BNN)                & 59.84          & 71.03            & 57.01           & \textbf{68.68}     & 82.67          & 87.54            \\
SiCF(mean+BNN)           & 59.91          & \textbf{71.10}   & 57.03           & 68.67              & 83.08          & \textbf{87.92}   \\
\hline
SiCF(mean+BNN, search)           &59.98	&71.20	&57.06	&68.75	&83.19	&87.99   \\
Pseudo oracle            & 61.63          & 72.98            & 58.41           & 70.35              & 85.49          & 90.32           \\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
    \caption{Uncertainty estimation results of SiCF score three datasets (SAMSUM 5:50, DIALOGSUM 5:50 and TODSUM 10:90) in terms of Rouge-1. } 
    \label{tab:uncertainty_R1_5p}
    \centering
    \scriptsize
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{Rouge-1} & \multicolumn{2}{c|}{SAMSUM (5:50)} & \multicolumn{2}{c|}{DIALOGSUM (5:50)} & \multicolumn{2}{c}{TODSUM (10:90)} \\
                         & 0-50\% mean    & 0-90\% mean      & 0-50\% mean     & 0-90\% mean        & 0-50\% mean    & 0-90\% mean      \\ \hline
Random rank                                    & 60.40                            & 70.97                            & 58.05                            & 69.18                            & 84.98                            & 88.99                            \\
SiCF(mean)                                     & 61.50                            & 72.24                            & 58.63                            & 69.85                            & 85.87                            & 89.92                            \\
SiCF(BNN)                                      & 61.71                            & 72.44                            & 58.61                            & \textbf{69.86}                   & 85.55                            & 89.67                            \\
SiCF(mean+BNN)                                 & 61.74                            & \textbf{72.45}                   & 58.64                            & 69.88                            & 85.83                            & \textbf{89.94}                   \\
\hline
SiCF(mean+BNN, search)           &61.86	&72.61	&58.70	&69.96	&85.84	&89.95   \\
Pseudo oracle                                  & 63.56                            & 74.41                            & 60.22                            & 71.66                            & 88.23                            & 92.30         
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
    \caption{Uncertainty estimation results of SiCF score three datasets (SAMSUM 1:50, DIALOGSUM 1:50 and TODSUM 2:90) in terms of BERTScore-F. } 
    \label{tab:uncertainty_BertF_1p}
    \centering
    \scriptsize
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{BERTScore-F} & \multicolumn{2}{c|}{SAMSUM (1:50)} & \multicolumn{2}{c|}{DIALOGSUM (1:50)} & \multicolumn{2}{c}{TODSUM (2:90)} \\
                         & 0-50\% mean    & 0-90\% mean      & 0-50\% mean     & 0-90\% mean        & 0-50\% mean    & 0-90\% mean      \\ \hline
Random rank                                        & 0.5792                           & 0.6913                           & 0.5803                           & 0.6921                           & 0.7766                           & 0.8365                           \\
SiCF(mean)                                         & 0.5890                           & 0.7028                           & 0.5885                           & 0.7008                           & 0.7878                           & 0.8480                           \\
SiCF(BNN)                                          & 0.5934                           & 0.7064                           & 0.5957                           & \textbf{0.7082}                  & 0.7851                           & 0.8464                           \\
SiCF(mean+BNN)                                     & 0.5938                           & \textbf{0.7069}                  & 0.5925                           & 0.7046                           & 0.7885                           & \textbf{0.8491}                  \\
\hline
SiCF(mean+BNN, search)           &0.5947	&0.7078	&0.5937	&0.7061	&0.7895	&0.8497   \\
Pseudo oracle                                      & 0.6135                           & 0.7288                           & 0.6159                           & 0.7298                           & 0.8156                           & 0.8770     
\\
\hline
\end{tabular}
\end{table*}













% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}
    \caption{Uncertainty estimation results of SiCF score three datasets (SAMSUM 5:50, DIALOGSUM 5:50 and TODSUM 10:90) in terms of BERTScore-F. } 
    \label{tab:uncertainty_BertF_5p}
    \centering
    \scriptsize
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{BERTScore-F} & \multicolumn{2}{c|}{SAMSUM (5:50)} & \multicolumn{2}{c|}{DIALOGSUM (5:50)} & \multicolumn{2}{c}{TODSUM (10:90)} \\
                         & 0-50\% mean    & 0-90\% mean      & 0-50\% mean     & 0-90\% mean        & 0-50\% mean    & 0-90\% mean      \\ \hline
Random rank                                        & 0.5939                           & 0.7021                           & 0.5946                           & 0.7024                           & 0.8105                           & 0.8611                           \\
SiCF(mean)                                         & 0.6045                           & 0.7144                           & 0.6042                           & 0.7129                           & 0.8205                           & 0.8717                           \\
SiCF(BNN)                                          & 0.6087                           & \textbf{0.7180}                  & 0.6103                           & \textbf{0.7193}                  & 0.8208                           & 0.8727                           \\
SiCF(mean+BNN)                                     & 0.6080                           & \textbf{0.7174}                  & 0.6078                           & 0.7168                           & 0.8223                           & \textbf{0.8738}                  \\
\hline
SiCF(mean+BNN, search)           &0.6095	&0.7189	&0.6074	&0.7168	&0.8227	&0.8743   \\
Pseudo oracle                                      & 0.6295                           & 0.7407                           & 0.6298                           & 0.7400                           & 0.8498                           & 0.9016        
\\
\hline
\end{tabular}
\end{table*}


% below is for the tables
\begin{table*}[]
    \caption{SSDS results on SAMSUM 1:50. } 
    \label{tab:ssds_samsum_1_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & 43.90                                               & 18.49                                               & 35.02                                               & 0.4374                                                  \\
Use all            & 1                                                        & 44.32                                               & 19.07                                               & 35.43                                               & 0.4372                                                  \\
\hline
Random rank        & 0.5                                                      & 45.16                                               & 19.47                                               & 35.59                                               & 0.4442                                                  \\
SiCF (mean)        & 0.5                                                      & 44.98                                               & 19.25                                               & 34.98                                               & 0.4385                                                  \\
SiCF (BNN)         & 0.5                                                      & 45.07                                               & 19.18                                               & 34.95                                               & 0.4434                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 45.14                                               & 19.47                                               & 35.19                                               & 0.4440                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                      & 45.05	&19.15	&35.12	&0.4442                                                  \\
Pseudo oracle      & 0.5                                                      & 45.58                                               & 19.79                                               & 35.95                                               & 0.4400                                                  \\
\hline
Random rank        & 0.25                                                     & 44.98                                               & 19.32                                               & 35.65                                               & 0.4439                                                  \\
SiCF (mean)        & 0.25                                                     & 45.85                                               & 19.90                                               & 35.96                                               & 0.4489                                                  \\
SiCF (BNN)         & 0.25                                                     & 45.20                                               & 19.95                                               & 35.63                                               & 0.4445                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 45.14                                               & 19.31                                               & 35.59                                               & 0.4447                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 45.40	&19.38	&35.48	&0.4434                                                  \\
Pseudo oracle      & 0.25                                                     & 44.92                                               & 19.87                                               & 35.67                                               & 0.4432   
\\                                             \hline 
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on SAMSUM 5:50. } 
    \label{tab:ssds_samsum_5_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & { 46.81}                        & { 20.46}                        & { 36.38}                        & { 0.4574}                           \\
Use all            & 1                                                        & { 47.76}                        & { 21.84}                        & { 38.20}                        & { 0.4702}                           \\
\hline
Random rank        & 0.5                                                      & 47.87                                               & 21.19                                               & 37.33                                               & 0.4677                                                  \\
SiCF (mean)        & 0.5                                                      & 47.94                                               & 21.51                                               & 37.09                                               & 0.4648                                                  \\
SiCF (BNN)         & 0.5                                                      & 47.72                                               & 21.39                                               & 37.46                                               & 0.4653                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 47.98                                               & 21.77                                               & 37.72                                               & 0.4704                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 48.23	& 21.83	&37.64	&0.4663                                              \\
Pseudo oracle      & 0.5                                                      & 48.40                                               & 21.73                                               & 38.16                                               & 0.4757                                                  \\
\hline
Random rank        & 0.25                                                     & 47.65                                               & 21.13                                               & 37.18                                               & 0.4666                                                  \\
SiCF (mean)        & 0.25                                                     & 47.90                                               & 21.39                                               & 37.57                                               & 0.4651                                                  \\
SiCF (BNN)         & 0.25                                                     & 47.77                                               & 22.07                                               & 37.67                                               & 0.4635                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 48.14                                               & 22.05                                               & 37.63                                               & 0.4661                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 47.83	&21.40	&37.24	&0.4655                                                  \\
Pseudo oracle      & 0.25                                                     & 48.33                                               & 21.97                                               & 37.93                                               & 0.4732                                                 
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on DialogSUM 1:50. } 
    \label{tab:ssds_dialogsum_1_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
\hline
Initial fine-tuned & -                                                        & { 40.30}                        & { 14.53}                        & { 31.19}                        & { 0.4389}                           \\
Use all            & 1                                                        & { 39.22}                        & { 14.04}                        & { 30.50}                        & { 0.4349}                           \\
\hline
Random rank        & 0.5                                                      & 39.54                                               & 14.58                                               & 30.92                                               & 0.4401                                                  \\
SiCF (mean)        & 0.5                                                      & 40.09                                               & 14.71                                               & 31.08                                               & 0.4366                                                  \\
SiCF (BNN)         & 0.5                                                      & 40.30                                               & 14.84                                               & 31.35                                               & 0.4418                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 39.16                                               & 14.19                                               & 30.71                                               & 0.4415                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 39.61	&14.75	&31.25	&0.4422                                                  \\
Pseudo oracle      & 0.5                                                      & 40.37                                               & 14.54                                               & 31.44                                               & 0.4469                                                  \\
\hline
Random rank        & 0.25                                                     & 39.66                                               & 14.32                                               & 30.89                                               & 0.4365                                                  \\
SiCF (mean)        & 0.25                                                     & 39.56                                               & 14.18                                               & 31.02                                               & 0.4360                                                  \\
SiCF (BNN)         & 0.25                                                     & 39.48                                               & 14.27                                               & 31.26                                               & 0.4401                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 39.98                                               & 14.68                                               & 31.14                                               & 0.4392                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 39.90	&14.40	&31.44	&0.4434                                                  \\
Pseudo oracle      & 0.25                                                     & 40.44                                               & 14.98                                               & 31.73                                               & 0.4543                                               
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on DialogSUM 5:50. } 
    \label{tab:ssds_dialogsum_5_50}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & { 42.28}                        & { 15.61}                        & { 33.18}                        & { 0.4629}                           \\
Use all            & 1                                                        & { 41.61}                        & { 16.04}                        & { 33.25}                        & { 0.4612}                           \\
\hline
Random rank        & 0.5                                                      & 42.06                                               & 16.01                                               & 33.07                                               & 0.4614                                                  \\
SiCF (mean)        & 0.5                                                      & 41.15                                               & 15.86                                               & 32.71                                               & 0.4522                                                  \\
SiCF (BNN)         & 0.5                                                      & 41.89                                               & 15.81                                               & 33.43                                               & 0.4624                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 41.89                                               & 15.86                                               & 33.31                                               & 0.4582                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 42.33	&16.27	&33.54	&0.4649                                                  \\
Pseudo oracle      & 0.5                                                      & 42.44                                               & 16.37                                               & 33.80                                               & 0.4687                                                  \\
\hline
Random rank        & 0.25                                                     & 42.32                                               & 16.38                                               & 33.70                                               & 0.4607                                                  \\
SiCF (mean)        & 0.25                                                     & 41.77                                               & 15.87                                               & 32.79                                               & 0.4548                                                  \\
SiCF (BNN)         & 0.25                                                     & 42.00                                               & 15.95                                               & 33.47                                               & 0.4670                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 42.85                                               & 16.86                                               & 34.06                                               & 0.4645                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 43.02	&17.22	&34.32	&0.4702                                                  \\
Pseudo oracle      & 0.25                                                     & 42.71                                               & 16.10                                               & 33.77                                               & 0.4705                                       
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on TODSUM 2:90. } 
    \label{tab:ssds_todsum_2_90}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & { 76.60}                        & { 59.51}                        & { 67.87}                        & { 0.7002}                           \\
Use all            & 1                                                        & { 77.02}                        & { 59.86}                        & { 68.09}                        & { 0.7057}                           \\
\hline
Random rank        & 0.5                                                      & 77.12                                               & 60.07                                               & 68.63                                               & 0.7087                                                  \\
SiCF (mean)        & 0.5                                                      & 76.93                                               & 59.91                                               & 68.48                                               & 0.7084                                                  \\
SiCF (BNN)         & 0.5                                                      & 76.29                                               & 59.19                                               & 67.59                                               & 0.7009                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 77.06                                               & 60.78                                               & 69.10                                               & 0.7118                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 77.17	&60.39	&69.12	&0.7132                                                  \\
Pseudo oracle      & 0.5                                                      & 78.44                                               & 61.65                                               & 70.11                                               & 0.7237                                                  \\
\hline
Random rank        & 0.25                                                     & 76.91                                               & 59.43                                               & 68.29                                               & 0.7064                                                  \\
SiCF (mean)        & 0.25                                                     & 77.94                                               & 61.01                                               & 69.64                                               & 0.7172                                                  \\
SiCF (BNN)         & 0.25                                                     & 76.64                                               & 59.66                                               & 68.71                                               & 0.7053                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 77.01                                               & 59.92                                               & 69.01                                               & 0.7091                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 76.45	&59.46	&68.77	&0.7064                                                  \\
Pseudo oracle      & 0.25                                                     & 79.09                                               & 63.19                                               & 71.94                                               & 0.7396                                                 
\\
\hline
\end{tabular}
\end{table*}


% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
    \caption{SSDS results on TODSUM 10:90. } 
    \label{tab:ssds_todsum_10_90}
    \centering
\begin{tabular}{l|ccccc}
\hline
                   & \multicolumn{1}{l}{Select Ratio} & \multicolumn{1}{l}{Rouge-1} & \multicolumn{1}{l}{Rouge-2} & \multicolumn{1}{l}{Rouge-L} & \multicolumn{1}{l}{BERTScore-F} \\
Initial fine-tuned & -                                                        & 79.75                      & 64.69                        & 72.77                        & 0.7428                           \\
Use all            & 1                                                        & 80.00                        & 64.99                        & 73.08                        & 0.7430                           \\
\hline
Random rank        & 0.5                                                      & 80.18                                               & 65.47                                               & 73.46                                               & 0.7484                                                  \\
SiCF (mean)        & 0.5                                                      & 80.95                                               & 65.95                                               & 73.96                                               & 0.7538                                                  \\
SiCF (BNN)         & 0.5                                                      & 81.06                                               & 66.32                                               & 74.62                                               & 0.7563                                                  \\
SiCF (mean+BNN)    & 0.5                                                      & 80.76                                               & 66.29                                               & 74.29                                               & 0.7550                                                  \\
SiCF (mean+BNN, search)    & 0.5                                                     & 80.61	&66.25	&74.17	&0.754                                                  \\
Pseudo oracle      & 0.5                                                      & 82.49                                               & 68.48                                               & 76.40                                               & 0.7718                                                  \\
\hline
Random rank        & 0.25                                                     & 80.57                                               & 65.73                                               & 73.76                                               & 0.7513                                                  \\
SiCF (mean)        & 0.25                                                     & 81.08                                               & 66.70                                               & 74.48                                               & 0.7575                                                  \\
SiCF (BNN)         & 0.25                                                     & 82.01                                               & 67.90                                               & 75.95                                               & 0.7674                                                  \\
SiCF (mean+BNN)    & 0.25                                                     & 80.93                                               & 66.32                                               & 74.58                                               & 0.7578                                                  \\
SiCF (mean+BNN, search)    & 0.25                                                     & 81.22	&67.14	&75.16	&0.7615                                                  \\
Pseudo oracle      & 0.25                                                     & 83.43                                               & 70.10                                               & 77.43                                               & 0.7848                                                 
\\
\hline
\end{tabular}
\end{table*}




\begin{table*}[htb]
    \caption{Ablation study of three components in SAMSUM 1:50 in terms of BERTScore F. The organization is similar to Table~\ref{tab:ab_samsum_unc_R1_1p}.} 
    \label{tab:ab_samsum_unc_bertf_1p}
    \centering
    \small
\begin{tabular}{l|cc|cc|cc}
\hline
\multirow{2}{*}{BERTScore-F} & \multicolumn{2}{c|}{SiCF (Mean)}                                   & \multicolumn{2}{c|}{SiCF (BNN)}                                    & \multicolumn{2}{c}{SiCF (m+BNN)}                               \\
                         & \multicolumn{1}{l}{0-50\% mean} & \multicolumn{1}{l|}{0-90\% mean} & \multicolumn{1}{l}{0-50\% mean} & \multicolumn{1}{l|}{0-90\% mean} & \multicolumn{1}{l}{0-50\% mean} & \multicolumn{1}{l}{0-90\% mean} \\
                         \hline
sein+cov+fai & \bf59.250$\pm$0.203  & \bf70.582$\pm$0.177 & \bf59.351$\pm$0.005 & \bf70.638$\pm$0.002 & \bf59.433$\pm$0.032 & \bf70.754$\pm$0.036 \\
only sein    & 58.826$\pm$0.001 & 70.143$\pm$0.000   & 58.826$\pm$0.001 & 70.143$\pm$0.000   & 58.826$\pm$0.001 & 70.143$\pm$0.000   \\
only cov     & 59.208$\pm$0.001 & 70.558$\pm$0.001 & 59.261$\pm$0.000   & 70.517$\pm$0.000   & 59.320$\pm$0.001  & 70.628$\pm$0.000   \\
only fai     & 58.080$\pm$0.039  & 69.402$\pm$0.049 & 59.062$\pm$0.000   & 70.307$\pm$0.000   & 58.610$\pm$0.000    & 69.694$\pm$0.000     
\\
\hline
\end{tabular}
\end{table*}


\begin{table}[!htb]
    \caption{SSDS results on DIALOGSUM 5:50 settings.  
    The values in the brackets are SSDS improved ratios. ROUGE-1 and ROUGE-L are listed in Table~\ref{tab:ssds_DIALOGSUM_wiL}. We do not report SSDS results on DIALOGSUM 1:50, as its generated pseudolabels are too noisy for training.
    % which indicates the improved degree compared to pseudo oracle. A SSDS improved ratio = (a method's metric score - initial finie-tuned's metric score) / (pseudo oracle's metric score - initial finie-tuned's metric score) $\times$ 100\%.
    } 
    \label{tab:ssds_dilogsum_medium}
    \centering
    \small
\begin{tabular}{l|cc}
\hline
\multirow{2}{*}{}  & \multicolumn{2}{c}{Medium-Size Labeled Data} \\
\cline{2-3}
                   & {ROUGE-2}  & {BERTScore-F}  \\
\hline
\hline
\multicolumn{3}{c}{DIALOGSUM}
\\
\hline
Initial Fine-Tuned                                                          & 15.61(0\%)   & 46.29(0\%)          \\
\hline
Full Unlabeled                                                                       & 16.04(87\%)    & 46.12(-22\%)           \\
% \hline
% Random Rank        & 0.5                                                      & 39.54                                               & 14.58                                               & 30.92                                               & 0.4401                                              & 42.06                                               & 16.01                                               & 33.07                                               & 0.4614    \\
% SiCF (mean)        & 0.5                                                      & 40.09                                               & 14.71                                               & 31.08                                               & 0.4366    & 41.15                                               & 15.86                                               & 32.71                                               & 0.4522                                               \\
% SiCF (BNN)         & 0.5                                                      & 40.30                                               & 14.84                                               & 31.35                                               & 0.4418    & 41.89                                               & 15.81                                               & 33.43                                               & 0.4624                                              \\
% SiCF (m+BNN)    & 0.5                                                      & 39.16                                               & 14.19                                               & 30.71                                               & 0.4415    & 41.89                                               & 15.86                                               & 33.31                                               & 0.4582                                                 \\
% SiCF (m+BNN-s)    & 0.5                                                     & 39.61	&14.75	&31.25	&0.4422    & 42.33	&16.27	&33.54	&0.4649                                              \\
% Pseudo Oracle      & 0.5                                                      & 40.37                                               & 14.54                                               & 31.44                                               & 0.4469      & 42.44                                               & 16.37                                               & 33.80                                               & 0.4687                                            \\
% \hline
Random Rank                                                                 & 16.38(157\%)    & 46.07(-28\%)  \\
SiCF (mean)                                                                 & 15.87(53\%)    & 45.48(-106\%)                                               \\
SiCF (BNN)                                                                & 15.95(69\%)   & 46.70(53\%)                                                \\
SiCF (m+BNN)                                                             & 16.86(255\%)   & 46.45(21\%)                                               \\
SiCF (m+BNN-s)                                                            & \bf{17.22}(\bf{328\%)}   & \bf{47.02}(\bf{96\%)} 
                                       \\
\hline
Pseudo Oracle                                                              & 16.10(100\%)   & 47.05(100\%)                                             
\\
\hline



\end{tabular}
\end{table}
